High-dimensional Berry-Esseen Bound for $m$-Dependent Random Samples

In this work, we provide a $(n/m)^{-1/2}$-rate finite sample Berry-Esseen bound for $m$-dependent high-dimensional random vectors over the class of hyper-rectangles. This bound imposes minimal assumptions on the random vectors such as nondegenerate covariances and finite third moments. The proof uses inductive relationships between anti-concentration inequalities and Berry--Esseen bounds, which are inspired by the telescoping method of Chen and Shao (2004) and the recursion method of Kuchibhotla and Rinaldo (2020). Performing a dual induction based on the relationships, we obtain tight Berry-Esseen bounds for dependent samples.

==> archived/b_alternative_local_rate.tex <==
\section{Alternative local rate for temporary use}

\begin{theorem} \label{thm:local_consistency} Let
    \begin{equation}
        \norm{L_{II^C}}_{\infty,2} := \sup_{x: \norm{x}_2 = 1} \norm{L_{II^C} x}_\infty = \max\{\norm{L_{iI^C}}_2 : i \in I\}.
    \end{equation}
    and
    \begin{equation}
        \norm{L_{II^C}}_2 = \sup_{x: \norm{x}_2 = 1} \norm{L_{II^C} x}_2.
    \end{equation}
    With every assumption in \cref{thm:ell_2_alt} and an additional assumption that 
    \begin{equation}
        \lambda_2(\tilde{I}_{II}(w^*)) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d} +  \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right),
    \end{equation}
    the error of the target parameter $\Delta_I = \hat{w}_I - w_I^*$ satisfies
    % \item For a sample size $n \geq \frac{c_1 \sigma^2 \tr(L^\dag)}{\eta B^2}$, any estimator $\tilde{w}$ satisfies
    % \begin{equation}
    %     \sup_{w^* \in \mathcal{W}_B} \Exp\left[\norm{\tilde{w} - w^*}_L^2\right] \geq \frac{c_{1l}}{\eta} \sigma^2 \frac{d}{n}.
    % \end{equation}
    \begin{enumerate}[label=\roman*.]
        \item Basic inequality:
        \begin{equation}
            \norm*{h\left(\bar{\Delta}_I\right)}_{\tilde{\mathcal{I}}_{II}} \leq c_{5u} \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}}
        \end{equation}
       for some universal constant $c_{4u} > 0 $ with probability at least $1 - \frac{1}{d}$ where $h(\Delta_I) \in \reals^{d_I}$ is the element-wise evaluation of $h$ at $\Delta_I$.
        
        \item $\ell_2$ convergence: Let
        \begin{equation}
            \gamma := \sup_{x \in \reals^d\backslash\{0\}} \norm{x}^2_L / \norm{x}^2_{\mathcal{I}(w^*)} = \sup_{x \in \reals^d\backslash\{0\}} \norm{x}^2_{\mathcal{I}(w^*)^{+}} / \norm{x}^2_{L^{+}} \leq \frac{2 v_\text{max}}{\lambda_2(\mathcal{I}(w^*)) n}
        \end{equation}
        and
        \begin{equation}
            \zeta := \sup_{x \in \reals^d\backslash \mathrm{span}(\mathbf{1})} \norm{x}^2_{L_{II}} / \norm{x}^2_{\tilde{L}_{II}}
        \end{equation}
        where $\tilde{L}_{II} = L_{II} - L_{II^C}L_{I^CI^C}^{-1}L_{I^CI}$. Then,
        \begin{equation}\label{eq:local_ell_2}
                h(\norm*{\bar{\Delta}_I}_2)  
                \leq c'_{5u} \left\{\sqrt{\frac{\gamma\zeta}{\lambda_2(\tilde{\mathcal{I}}_{II})}\frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\lambda_2(\tilde{\mathcal{I}}_{II})} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}\\
        \end{equation}
        with probability at least $1-\frac{1}{d}-e^{-t}$ for some universal constant $c'_{5u} > 0$.
    \end{enumerate}
\end{theorem}
The proof is provided in \cref{sec:pf_local_consistency}.

\subsection{Proof of \cref{thm:local_consistency}} \label{sec:pf_local_consistency}
Bounding the size of $\bar{\Delta}_I$ from \cref{eq:local_quad_ineq} involves with bounding $\nabla_I l^*(\tilde{w})$. Our strategy is to approximate $\nabla_I l^*(\tilde{w})$ by $\nabla_I l^*(\hat{w})$ and then bound the difference. For each $i \in I$, the $i$-th element of the gradient difference is
\begin{equation}
\begin{split}
    \nabla_i l^*(\hat{w}) - \nabla_i l^*(\tilde{w}) 
    &= \frac{1}{n} \sum_k \left\{ \frac{x_{ik}+x_{ki}}{1+e^{\tilde{w}_k - \tilde{w}_i}} - \frac{x_{ik}+x_{ki}}{1+e^{\hat{w}_k - \hat{w}_i}}\right\} \\
    &= \frac{1}{n} \sum_{k \in I^C} \left\{ \frac{x_{ik}+x_{ki}}{1+e^{\tilde{w}_k - \hat{w}_i}} - \frac{x_{ik}+x_{ki}}{1+e^{\hat{w}_k - \hat{w}_i}}\right\}
\end{split}
\end{equation}
because $\hat{w}_I = \tilde{w}_I$. We bound the summand using the fact that $\abs{\frac{d}{dx}\frac{1}{1+e^{-x}}} \leq 1$. The resulting upperbound is
\begin{equation}
\begin{split}
    \abs{\nabla_i l^*(\hat{w}) - \nabla_i l^*(\tilde{w})}
    &\leq \frac{1}{n} \sum_{k \in I^C} (x_{ik}+x_{ki}) \abs{\hat{w}_k - \tilde{w}_k}.
\end{split}
\end{equation}
We notice that $\abs{\nabla_I l^*(\hat{w})}$ is elementwise upperbounded by $L_{II^C} \abs{\tilde{\Delta}_I - \Delta_I}$. This observation leads us to the following lemma and corollary. Their proofs are provided in \cref{sec:pf_lemmas}.
\begin{lemma}\label{lem:bound_grad_diff}
    Under $\lambda_2(\mathcal{I}(w^*)) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w}) - \nabla_I l^*(\tilde{w})}_\infty 
        \leq c_{A1} \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w}) - \nabla_I l^*(\tilde{w})}_2 
        \leq c_{A1}' \norm{L_{II^C}}_2 ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A1}$ and $c_{A1}'$.
\end{lemma}

\begin{lemma}\label{lem:bound_grad_hat}
    Under $\lambda_2(\mathcal{I}(w^*)) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w})}_\infty 
        \leq c_{A2} \frac{1}{n} \sqrt{v_\text{max} \log d}
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w})}_2 
        \leq c_{A2}' \sqrt{\gamma \zeta \frac{td_I}{n}}
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A2}$ and $c_{A2}'$.
\end{lemma}

The above two lemmas result into the following corollary.
\begin{corollary}\label{cor:bound_grad_tilde}
Under $\lambda_2(\mathcal{I}(w^*)) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\tilde{w})}_\infty 
        \leq c_{A3} \left\{ \frac{1}{n} \sqrt{v_\text{max} \log d} +  \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right) \right\}
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} 
        \leq c_{A3}' \left\{\sqrt{\gamma \zeta \frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\sqrt{\lambda_2(\tilde{\mathcal{I}}_{II})}} ~h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A3}$ and $c_{A3}'$.
\end{corollary}

According to the corollary, the given condition of $\lambda_2(\tilde{\mathcal{I}}_{II})$ guarantees $\lambda_2(\tilde{\mathcal{I}}_{II}) \gtrsim \norm{\nabla_I l^*(\tilde{w})}_\infty$ with high probability. Then, the same argument as in \cref{sec:alternative_l2} establishes
\begin{equation}
    \norm{h(\bar{\Delta}_I)}_{\tilde{\mathcal{I}}_{II}} \lesssim \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} \leq c_{A3}' \left\{\sqrt{\gamma \zeta \frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\sqrt{\lambda_2(\tilde{\mathcal{I}}_{II})}} ~h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}.
\end{equation}
with probability at least $1 - e^{-t}-\frac{1}{d}$ for sufficiently large $d$. The rest of the proof is a straightforward application of our argument in the previous paper.

\subsection{Proofs of lemmas} \label{sec:pf_lemmas}

\subsubsection{Proof of \cref{lem:bound_grad_diff}}

We recall the original basic inequality in the previous paper, which implies
\begin{equation}
    l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*) \leq \Delta^\top \nabla l(w^*)
\end{equation}
because of the optimality of $\tilde{w}$ in \cref{eq:tilde_optimality}. Provided that $\lambda_2(\mathcal{I}(w^*)) \gtrsim \frac{1}{n}\sqrt{v_\mathrm{max} \log d}$, $\lambda_2(\mathcal{I}(w^*)) \geq 4 c_{3u} \norm{\nabla l(w^*)}_\infty$ for $c_{3u} > 0$ in \cref{eq:quad_ineq} with probability at least $1-\frac{1}{d}$ for sufficiently large $d$. Hence, by \cref{eq:quad_ineq_by_h},
\begin{equation}
\begin{split}
    &l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*)  \\ 
    &\leq 2 c_{3u}\left\{h(\Delta)^\top \nabla l(w^*) +
    \norm{\nabla l(w^*)}_\infty h(\Delta)^\top \left(I - \frac{1}{d} \mathbf{1}\mathbf{1}^\top \right) h(\Delta) \right\} \\
    &\leq 2 c_{3u} h(\Delta)^\top \nabla l(w^*) +
     \frac{1}{2} h(\Delta)^\top \mathcal{I}(w^*) h(\Delta),
\end{split}
\end{equation}
and \cref{thm:ell_2_alt} establishes
\begin{equation}
\begin{split}
    &l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*)
    \leq c \norm{\nabla l(w^*)}_{\mathcal{I}(w^*)^{+}}.
\end{split}
\end{equation}
for a universal constant $c = 2c_{3u}c_{4u} + \frac{1}{2}c_{4u}^2$. Then, Hanson-Wright inequality gives
\begin{equation}
    l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*) 
    \leq c' \gamma \frac{td}{n}
\end{equation}
with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c' > 0$. This implies two inequalities, one about $\tilde{\Delta} = \tilde{w} - w^*$ and the other about $\Delta = \hat{w} - w^*$:
\begin{equation}
    h(\tilde{\Delta})^\top \mathcal{I}(w^*) h(\tilde{\Delta}) \leq l^*(\tilde{w}) - l^*(w^*)
    \leq c' \gamma \frac{td}{n}
\end{equation}
and
\begin{equation}
    h(\Delta)^\top \mathcal{I}(w^*) h(\Delta) \leq l^*(\hat{w}) - l^*(w^*)
    \leq c' \gamma \frac{td}{n}.
\end{equation}
Thus, we obtain the bound on $\tilde{\Delta}$ and $\Delta$ as follows:
\begin{equation}
    \norm{\tilde{\Delta}}_2, \norm{\Delta}_2 \leq c'' \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I}(w^*))}\frac{td}{n}}
\end{equation}
for some universal constant $c'' > 0$, and 
\begin{equation}
    \norm{\tilde{\Delta}-\Delta}_2 \leq 2c'' \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I}(w^*))}\frac{td}{n}}.
\end{equation}
Then, the desired result immediately follows, based on the definition of $\norm{L_{II^C}}_2$ and $\norm{L_{II^C}}_{\infty,2}$.

\subsubsection{Proof of \cref{cor:bound_grad_tilde}}

The upperbound of $\norm{\nabla_I l(w^*)}_\infty$ is the direct result of the maximal inequality on sub-Gaussian random variables \citep{wainwright2019high}. For the upperbound of $\norm{\nabla_I l(w^*)}_2$, we introduce the following lemma.
\begin{lemma}\label{lem:equiv_L_and_I}
\begin{equation}
    \sup_{x \in \reals^{d_I}\backslash\{0\}} \norm{x}^2_{\tilde{L}_{II}} / \norm{x}^2_{\tilde{\mathcal{I}}_{II}} \leq \gamma
\end{equation}
\end{lemma}
The proof is provided in \cref{sec:pf_equiv_L_and_I}. Based on the lemma,
\begin{equation}
\begin{split}
    \norm{\nabla_I l(w^*)}_{\tilde{\mathcal{I}}_{II}^{+}}
    &\leq \sqrt{\gamma} \norm{\nabla_I l(w^*)}_{\tilde{L}_{II}^{+}} \\
    &\leq \sqrt{\gamma\zeta} \norm*{\left(I - \frac{1}{d_I} \mathbf{1}\mathbf{1}^\top\right) \nabla_I l(w^*)}_{L_{II}^{-1}} \\
    &\leq \sqrt{\gamma\zeta} \norm*{\nabla_I l(w^*)}_{L_{II}^{-1}},
\end{split}
\end{equation}
and the Hanson-Wright inequality establishes
\begin{equation}
    \norm{\nabla_I l(w^*)}_{\tilde{\mathcal{I}}_{II}^{+}} \leq \sqrt{\gamma\zeta\frac{td_I}{n}} 
\end{equation}
with probability at least $1 - e^{-t}$.

\subsubsection{Proof of \cref{lem:equiv_L_and_I}} \label{sec:pf_equiv_L_and_I}

TODO

==> archived/b_auxiliary.tex <==
\section{Alternative local rate for temporary use}

\begin{theorem} \label{thm:local_consistency_2} Let
    \begin{equation}
        \norm{L_{II^C}}_{\infty,2} := \sup_{x: \norm{x}_2 = 1} \norm{L_{II^C} x}_\infty = \max\{\norm{L_{iI^C}}_2 : i \in I\}.
    \end{equation}
    and
    \begin{equation}
        \norm{L_{II^C}}_2 = \sup_{x: \norm{x}_2 = 1} \norm{L_{II^C} x}_2.
    \end{equation}
    With every assumption in \cref{thm:ell_2_alt} and an additional assumption that 
    \begin{equation}
        \lambda_2(\tilde{\mathcal{I}}_{II}) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d} +  \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right),
    \end{equation}
    the error of the target parameter $\Delta_I = \hat{w}_I - w_I^*$ satisfies
    % \item For a sample size $n \geq \frac{c_1 \sigma^2 \tr(L^\dag)}{\eta B^2}$, any estimator $\tilde{w}$ satisfies
    % \begin{equation}
    %     \sup_{w^* \in \mathcal{W}_B} \Exp\left[\norm{\tilde{w} - w^*}_L^2\right] \geq \frac{c_{1l}}{\eta} \sigma^2 \frac{d}{n}.
    % \end{equation}
    \begin{enumerate}[label=\roman*.]
        \item Basic inequality:
        \begin{equation}
            \norm*{h\left(\bar{\Delta}_I\right)}_{\tilde{\mathcal{I}}_{II}} \leq c_{5u} \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}}
        \end{equation}
       for some universal constant $c_{4u} > 0 $ with probability at least $1 - \frac{1}{d}$ where $h(\Delta_I) \in \reals^{d_I}$ is the element-wise evaluation of $h$ at $\Delta_I$.
        
        \item $\ell_2$ convergence: Let
        \begin{equation}
            \gamma := \sup_{x \in \reals^d\backslash\{0\}} \norm{x}^2_L / \norm{x}^2_{\mathcal{I}} = \sup_{x \in \reals^d\backslash\{0\}} \norm{x}^2_{\mathcal{I}^{+}} / \norm{x}^2_{L^{+}} \leq \frac{2 v_\text{max}}{\lambda_2(\mathcal{I}) n}.
        \end{equation}
        % and
        % \begin{equation}
        %     \zeta := \sup_{x \in \reals^d\backslash \mathrm{span}(\mathbf{1})} \norm{x}^2_{L_{II}} / \norm{x}^2_{\tilde{L}_{II}}
        % \end{equation}
        % where $\tilde{L}_{II} = L_{II} - L_{II^C}L_{I^CI^C}^{-1}L_{I^CI}$. 
        Then,
        \begin{equation}\label{eq:local_ell_2_2}
            h(\norm*{\bar{\Delta}_I}_2)  
            \leq c'_{5u} \left\{\sqrt{\frac{\gamma}{\lambda_2(\tilde{\mathcal{I}}_{II})}\frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\lambda_2(\tilde{\mathcal{I}}_{II})} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}\\
        \end{equation}
        with probability at least $1-\frac{1}{d}-e^{-t}$ for some universal constant $c'_{5u} > 0$.
    \end{enumerate}
\end{theorem}

\subsection{Proof}

Bounding the size of $\bar{\Delta}_I$ from \cref{eq:local_quad_ineq} involves with bounding $\nabla_I l^*(\tilde{w})$. Our strategy is to approximate $\nabla_I l^*(\tilde{w})$ by $\nabla_I l^*(\hat{w})$ and then bound the difference. For each $i \in I$, the $i$-th element of the gradient difference is
\begin{equation}
\begin{split}
    \nabla_i l^*(\hat{w}) - \nabla_i l^*(\tilde{w}) 
    &= \frac{1}{n} \sum_k \left\{ \frac{x_{ik}+x_{ki}}{1+e^{\tilde{w}_k - \tilde{w}_i}} - \frac{x_{ik}+x_{ki}}{1+e^{\hat{w}_k - \hat{w}_i}}\right\} \\
    &= \frac{1}{n} \sum_{k \in I^C} \left\{ \frac{x_{ik}+x_{ki}}{1+e^{\tilde{w}_k - \hat{w}_i}} - \frac{x_{ik}+x_{ki}}{1+e^{\hat{w}_k - \hat{w}_i}}\right\}
\end{split}
\end{equation}
because $\hat{w}_I = \tilde{w}_I$. We bound the summand using the fact that $\abs{\frac{d}{dx}\frac{1}{1+e^{-x}}} \leq 1$. The resulting upperbound is
\begin{equation}
\begin{split}
    \abs{\nabla_i l^*(\hat{w}) - \nabla_i l^*(\tilde{w})}
    &\leq \frac{1}{n} \sum_{k \in I^C} (x_{ik}+x_{ki}) \abs{\hat{w}_k - \tilde{w}_k}.
\end{split}
\end{equation}
We notice that $\abs{\nabla_I l^*(\hat{w})}$ is elementwise upperbounded by $L_{II^C} \abs{\tilde{\Delta}_I - \Delta_I}$. This observation leads us to the following lemma and corollary. Their proofs are provided in \cref{sec:pf_lemmas}.
\begin{lemma}\label{lem:bound_grad_diff_2}
    Under $\lambda_2(\mathcal{I}) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w}) - \nabla_I l^*(\tilde{w})}_\infty 
        \leq c_{A1} \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w}) - \nabla_I l^*(\tilde{w})}_2
        \leq c_{A1}' \norm{L_{II^C}}_2 ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A1}$ and $c_{A1}'$.
\end{lemma}

\begin{lemma}\label{lem:bound_grad_hat_2}
    Under $\lambda_2(\mathcal{I}) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w})}_\infty 
        \leq c_{A2} \frac{1}{n} \sqrt{v_\text{max} \log d}
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\hat{w}) - L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} 
        \leq c_{A2}' \sqrt{\gamma\frac{td_I}{n}}
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A2}$ and $c_{A2}'$.
\end{lemma}

The above two lemmas result into the following corollary.
\begin{corollary}\label{cor:bound_grad_tilde_2}
Under $\lambda_2(\mathcal{I}) \gtrsim \frac{1}{n} \sqrt{v_\text{max} \log d}$, both
    \begin{equation}
        \norm{\nabla_I l^*(\tilde{w})}_\infty 
        \leq c_{A3} \left\{ \frac{1}{n} \sqrt{v_\text{max} \log d} +  \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right) \right\}
    \end{equation}
    and
    \begin{equation}
        \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} 
        \leq c_{A3}' \left\{\sqrt{\gamma \frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\sqrt{\lambda_2(\tilde{\mathcal{I}}_{II})}} ~h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}
    \end{equation}
    hold simultaneously with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c_{A3}$ and $c_{A3}'$.
\end{corollary}

According to the corollary, the given condition of $\lambda_2(\tilde{\mathcal{I}}_{II})$ guarantees $\lambda_2(\tilde{\mathcal{I}}_{II}) \gtrsim \norm{\nabla_I l^*(\tilde{w})}_\infty$ with high probability. Then, the same argument as in \cref{sec:alternative_l2} establishes
\begin{equation}
    \norm{h(\bar{\Delta}_I)}_{\tilde{\mathcal{I}}_{II}} \lesssim \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} \leq c_{A3}' \left\{\sqrt{\gamma \frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\sqrt{\lambda_2(\tilde{\mathcal{I}}_{II})}} ~h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}.
\end{equation}
with probability at least $1 - e^{-t}-\frac{1}{d}$ for sufficiently large $d$. The rest of the proof is a straightforward application of our argument in the previous paper.

\subsection{Proofs of lemmas}

\subsubsection{Proof of \cref{lem:bound_grad_diff_2}}

We recall the original basic inequality in the previous paper, which implies
\begin{equation}
    l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*) \leq \Delta^\top \nabla l(w^*)
\end{equation}
because of the optimality of $\tilde{w}$ in \cref{eq:tilde_optimality}. Provided that $\lambda_2(\mathcal{I}) \gtrsim \frac{1}{n}\sqrt{v_\mathrm{max} \log d}$, $\lambda_2(\mathcal{I}) \geq 4 c_{3u} \norm{\nabla l(w^*)}_\infty$ for $c_{3u} > 0$ in \cref{eq:quad_ineq} with probability at least $1-\frac{1}{d}$ for sufficiently large $d$. Hence, by \cref{eq:quad_ineq_by_h},
\begin{equation}
\begin{split}
    &l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*)  \\ 
    &\leq 2 c_{3u}\left\{h(\Delta)^\top \nabla l(w^*) +
    \norm{\nabla l(w^*)}_\infty h(\Delta)^\top \left(I - \frac{1}{d} \mathbf{1}\mathbf{1}^\top \right) h(\Delta) \right\} \\
    &\leq 2 c_{3u} h(\Delta)^\top \nabla l(w^*) +
     \frac{1}{2} h(\Delta)^\top \mathcal{I} ~ h(\Delta),
\end{split}
\end{equation}
and \cref{thm:ell_2_alt} establishes
\begin{equation}
\begin{split}
    &l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*)
    \leq c \norm{\nabla l(w^*)}_{\mathcal{I}(w^*)^{+}}.
\end{split}
\end{equation}
for universal constant $c = 2c_{3u}c_{4u} + \frac{1}{2}c_{4u}^2$. Then, Hanson-Wright inequality gives
\begin{equation}
    l^*(\tilde{w}) - l^*(w^*) \leq l^*(\hat{w}) - l^*(w^*) 
    \leq c' \gamma \frac{td}{n}
\end{equation}
with probability at least $1 - e^{-t} - \frac{1}{d}$ for some universal constant $c' > 0$. This implies two inequalities, one about $\tilde{\Delta} = \tilde{w} - w^*$ and the other about $\Delta = \hat{w} - w^*$:
\begin{equation}
    h(\tilde{\Delta})^\top \mathcal{I} ~ h(\tilde{\Delta}) \leq l^*(\tilde{w}) - l^*(w^*)
    \leq c' \gamma \frac{td}{n}
\end{equation}
and
\begin{equation}
    h(\Delta)^\top \mathcal{I} ~ h(\Delta) \leq l^*(\hat{w}) - l^*(w^*)
    \leq c' \gamma \frac{td}{n}.
\end{equation}
Thus, we obtain the bound on $\tilde{\Delta}$ and $\Delta$ as follows:
\begin{equation}
    \norm{\tilde{\Delta}}_2, \norm{\Delta}_2 \leq c'' h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})}\frac{td}{n}}\right)
\end{equation}
for some universal constant $c'' > 0$, and 
\begin{equation}
    \norm{\tilde{\Delta}-\Delta}_2 \leq 2c'' h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})}\frac{td}{n}}\right).
\end{equation}
Then, the desired result immediately follows based on the definition of $\norm{L_{II^C}}_2$ and $\norm{L_{II^C}}_{\infty,2}$.

\subsubsection{Proof of \cref{lem:bound_grad_hat_2}}

The upperbound of $\norm{\nabla_I l(w^*)}_\infty$ is the direct result of the maximal inequality on sub-Gaussian random variables \citep{wainwright2019high}. For the upperbound of $\norm{\nabla_I l(w^*)}_2$, we introduce the following lemma.
\begin{lemma}\label{lem:equiv_L_and_I_2}
\begin{equation}
    \sup_{x \in \reals^{d_I}\backslash\{0\}} \norm{x}^2_{\tilde{L}_{II}} / \norm{x}^2_{\tilde{\mathcal{I}}_{II}} \leq \gamma
\end{equation}
\end{lemma}
The proof is provided in \cref{sec:pf_equiv_L_and_I}. Based on the lemma,
\begin{equation}
\begin{split}
    &\norm{\nabla_I l^*(\hat{w}) - L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} \\
    &\leq \sqrt{\gamma} \norm{\nabla_I l^*(\hat{w}) - L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\tilde{L}_{II}^{+}} \\
    % &\leq \sqrt{\gamma\zeta} \norm*{\left(I - \frac{1}{d_I} \mathbf{1}\mathbf{1}^\top\right) \nabla_I l(w^*)}_{L_{II}^{-1}} \\
    % &\leq \sqrt{\gamma\zeta} \norm*{\nabla_I l(w^*)}_{L_{II}^{-1}},
\end{split}
\end{equation}
and the Hanson-Wright inequality establishes \commhb{Need more explanation}
\begin{equation}
    \norm{\nabla_I l(w^*)}_{\tilde{\mathcal{I}}_{II}^{+}} \leq \sqrt{\gamma\frac{td_I}{n}} 
\end{equation}
with probability at least $1 - e^{-t}$.

\subsubsection{Proof of \cref{cor:bound_grad_tilde_2}} 

We first note that
\begin{equation}
    \nabla_i l^*(\hat{w}) = \sum_j \left\{\frac{x_{ij}+x_{ji}}{1+e^{w^*_j - w^*_i} - \frac{x_{ij}+x_{ji}}{1+e^{\hat{w}_j - \hat{w}_i}}}\right\} = - \nabla_i l(w^*)
\end{equation}
for $i=1,\dots,d$. Then, for the $\ell_\infty$ norm,
\begin{equation}
\begin{split}
    &\norm{\nabla_I l^*(\tilde{w})}_\infty \leq \norm{\nabla_I l(w^*)}_\infty + \norm{\nabla_I l^*(\hat{w}) - \nabla_I l^*(\tilde{w})}_\infty \\
    &\leq c_{A3} \left\{ \frac{1}{n} \sqrt{v_\text{max} \log d} +  \norm{L_{II^C}}_{\infty, 2} ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right) \right\}
\end{split}
\end{equation}
for some universal constant $c_{A3}$.

For the $\tilde{I}_{II}^{+}$ norm, we need an upperbound for $\norm{L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}}$. We first observe that
\begin{equation}
\begin{split}
    & \norm{L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\hat{\mathcal{I}}_{II}^{+}} \\
    & \leq \sqrt{\gamma} \norm{L_{II^C} L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\tilde{w})}_{\hat{L}_{II}^{+}} \\
    & \leq \sqrt{\gamma} \norm{L_{I^CI^C}^{-1/2} \nabla_{I^C} l^*(\tilde{w})}_{\mathcal{A}}
\end{split}
\end{equation}
where $\mathcal{A} = L_{I^CI^C}^{-1/2} L_{I^CI} \tilde{L}_{II}^{+} L_{II^C} L_{I^CI^C}^{-1/2}$. Then,
\begin{equation}
\begin{split}
    \norm{L_{I^CI^C}^{-1/2} \nabla_{I^C} l^*(\hat{w})}_{\mathcal{A}} \leq \norm{\mathcal{A}}_2 \norm{\nabla_{I^C} l^*(\hat{w})}_{L_{I^CI^C}^{-1}}.
\end{split}
\end{equation}
By the Hanson-Wright inequality, \commhb{Need more explanation}
\begin{equation}
    \norm{\nabla_{I^C} l^*(\tilde{w})}_{L_{I^CI^C}^{-1}} \leq c \sqrt{\frac{td_{I^C}}{n}}
\end{equation}
with probability at least $1 - e^{-t}$ for some universal constant $c$. In sum,
\begin{equation}
\begin{split}
    & \norm{\nabla_I l^*(\tilde{w})}_{\tilde{\mathcal{I}}_{II}^{+}} \leq \norm{\nabla_I l^*(\hat{w}) - L_{II^C}L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\hat{w})}_{\tilde{\mathcal{I}}_{II}^{+}} + \norm{\nabla_I l^*(\tilde{w}) - \nabla_I l^*(\hat{w})}_{\tilde{\mathcal{I}}_{II}^{+}}  \\
    & + \norm{L_{II^C}L_{I^CI^C}^{-1} \nabla_{I^C} l^*(\hat{w})}_{\tilde{\mathcal{I}}_{II}^{+}} \\
    & \leq c_{A2}' \sqrt{\gamma\frac{td_I}{n}} + c \sqrt{\gamma} \norm{\mathcal{A}}_2 \sqrt{\frac{td_{I^C}}{n}} + c_{A1}' \norm{L_{II^C}}_2 ~h^{-1}\left( \sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right) \\
    & \leq c_{A3}' \left\{\sqrt{\gamma \frac{td_I}{n}} + \frac{\norm{L_{II^C}}_2}{\sqrt{\lambda_2(\tilde{\mathcal{I}}_{II})}} ~h^{-1}\left(\sqrt{\frac{\gamma}{\lambda_2(\mathcal{I})} \frac{td}{n}}\right)\right\}
\end{split}
\end{equation}
for some universal constant $c'_{A3}$.

==> sections/2_methods.tex <==
% \section{Assumptions} \label{sec:assumptions}



% \begin{itemize}
%     \item For $i,j : 1 \leq i \leq j \leq n$, let $\underline{\sigma}_{[i,j]}$ and $\overline{\sigma}_{[i,j]}$ be
%     \begin{equation}
%         \underline{\sigma}^2_{[i,j]} :=
%         % \mathrm{inf} \left\{\begin{aligned}
%         \lambda_{\min}(\Var[SX_{[i,j]}])
%         % & \lambda_{\min}(\Var[SY_{[i,j]}])
%         % \end{aligned}\right\}
%         \textand 
%         \overline{\sigma}^2_{[i,j]} :=
%         % \mathrm{inf} \left\{\begin{aligned}
%         \lambda_{\max}(\Var[SX_{[i,j]}]).
%         % & \lambda_{\max}(\Var[SY_{[i,j]}])
%         % \end{aligned}\right\}.
%     \end{equation}
%     We assume $\underline{\sigma}^2_{[i,j]} \geq \underline{\sigma}^2 \cdot (i-j+1) \cdot m$ and $\overline{\sigma}^2_{[i,j]} \leq \overline{\sigma}^2 \cdot (i-j+1) \cdot m$ for some $\underline{\sigma}, \overline{\sigma} > 0$.
    
%     \item For $i,j : 1 \leq i \leq j \leq n$, let $\underline{\sigma}_{[i,j]}$ be
%     \begin{equation}
%         {\sigma}^2_{\min,[i,j]} :=
%         % \mathrm{inf} \left\{\begin{aligned}
%         \min_{k \in [p]} \Var[SX^{(k)}_{[i,j]}].
%         % & \min_{k \in [p]} \Var[SY^{(k)}_{[i,j]}]
%         % \end{aligned}\right\}.
%     \end{equation}
%     We assume $\sigma^2_{\min,[i,j]} \geq \sigma^2_{\min} \cdot (i-j+1) \cdot m$ for some $\sigma_{\min} > 0$.
    
%     \item Let $\nu_{3}$ be
%     \begin{equation}
%         \nu_{3} :=
%         \mathrm{sup} \left\{\begin{aligned}
%         & \Exp[\norm{X_{i_1} \otimes X_{i_2} \otimes X_{i_3}}_\infty] \\ 
%         & \Exp[\norm{X_{i_1} \otimes X_{i_2} \otimes Y_{i_3}}_\infty] \\ 
%         & \Exp[\norm{X_{i_1} \otimes Y_{i_2} \otimes Y_{i_3}}_\infty] \\
%         & \Exp[\norm{Y_{i_1} \otimes Y_{i_2} \otimes Y_{i_3}}_\infty]
%         \end{aligned}:
%         1 \leq i_1, i_2, i_3 \leq n \right\} < \infty.
%     \end{equation}
% \end{itemize}





